AutoIOT: LLM-Driven Automated Natural Language Programming for AIoT Applications

The advent of Large Language Models (LLMs) has profoundly transformed our lives, revolutionizing interactions with AI and lowering the barrier to AI usage. While LLMs are primarily designed for natural language interaction, the extensive embedded knowledge empowers them to comprehend digital sensor data. This capability enables LLMs to engage with the physical world through IoT sensors and actuators, performing a myriad of AIoT tasks. Consequently, this evolution triggers a paradigm shift in conventional AIoT application development, democratizing its accessibility to all by facilitating the design and development of AIoT applications via natural language. However, some limitations need to be addressed to unlock the full potential of LLMs in AIoT application development. First, existing solutions often require transferring raw sensor data to LLM servers, which raises privacy concerns, incurs high query fees, and is limited by token size. Moreover, the reasoning processes of LLMs are opaque to users, making it difficult to verify the robustness and correctness of inference results. This paper introduces AutoIOT, an LLM-based automated program generator for AIoT applications. AutoIOT enables users to specify their requirements using natural language (input) and automatically synthesizes interpretable programs with documentation (output). AutoIOT automates the iterative optimization to enhance the quality of generated code with minimum user involvement. AutoIOT not only makes the execution of AIoT tasks more explainable but also mitigates privacy concerns and reduces token costs with local execution of synthesized programs. Extensive experiments and user studies demonstrate AutoIOT's remarkable capability in program synthesis for various AIoT tasks. The synthesized programs can match and even outperform some representative baselines.

==> sections/possibleConcerns.tex <==
\revise{How does the LLM detect a lack of relevant knowledge?}

\revise{More details should be presented about the construction of context database. Constructing knowledge dataset is a hot emerging area. Reviewers will have lots of concerns and questions}

\revise{I am afraid that many baselines (especially for HAR tasks) are not SOTAs. We may need to relax our claim a little bit. Actually, we do not need to compare AutoNLP to SOTA. It will be fine to demonstrate that AutoNLP can automatically generate the code with decent performance.}

\revise{How much testing data did you use for communication evaluation? We can imagine PenAI will be better than your system if only one ECG trace is tested. The same question goes to inference time. It would be interesting to see where the turning point is for these two metrics along with the data size. Moreover, why not compare the accuracy of PenAI to AutoNLP? You may also compare AutoNLP to existing tokenization methods, since they can also reduce the communication overhead to a great extent.} 

\revise{I believe there were cases where LLM got stuck and could not resolve a bug and the user had to intervene. Report some statistics can make this paper more down-to-earth.}

\revise{I think we can summarize the lessons learned in both the ECG task and the HAR task since the latter task also has many insightful analyses. Considering placing the lessons before 6.2.2.}
